Developing a Practical Reactive Synthesis Tool: Experience and Lessons Learned

We summarise our experience developing and using Termite, the first reactive synthesis tool intended for use by software development practitioners. We identify the main barriers to making reactive synthesis accessible to software developers and describe the key features of Termite designed to overcome these barriers, including an imperative C-like specification language, an interactive source-level debugger, and a user-guided code generator. Based on our experience applying Termite to synthesising real-world reactive software, we identify several caveats of the practical use of the reactive synthesis technology. We hope that these findings will help define the agenda for future research on practical reactive synthesis.

==> eptcsdata.tex <==
\providecommand{\firstpage}{84}
\providecommand{\publicationstatus}{Dimitrova, Piskac (Eds.): Fifth Workshop on\\ 
Synthesis (SYNT 2016)\\
EPTCS 229, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.229.8}{10.4204/EPTCS.229.8}}
\pdfoutput=1

